Sharing Heartbeats: Motivations of Citizen Scientists in Times of Crises

With the rise of COVID-19 cases globally, many countries released digital tools to mitigate the effects of the pandemic. In Germany the Robert Koch Institute (RKI) published the Corona-Data-Donation-App, a virtual citizen science (VCS) project, to establish an early warning system for the prediction of potential COVID-19 hotspots using data from wearable devices. While work on motivation for VCS projects in HCI often presents egoistic motives as prevailing, there is little research on such motives in crises situations. In this paper, we explore the socio-psychological processes and motivations to share personal data during a pandemic. Our findings indicate that collective motives dominated among app reviews (n=464) and in in-depth interviews (n=10). We contribute implications for future VCS tools in times of crises that highlight the importance of communication, transparency and responsibility.

==> TextFragements.tex <==


%\subsection{Themen für Intro}
%- crisis fatigue (in Review Daten ablesbar) %reference for crisis fatigue would be awesome. I only found blog articles for now
%- Downloadzahlen Corona-Data-Donation-App: 515.374 (Stand 2.6.2020; Datenspende App Blog)
%- Downloadzahlen Corona Tracing App: 14,6 Millionen (Stand 03.07.2020; %https://www.connect.de/news/corona-warn-app-download-zahlen-3200860.html)
% some autoethnographic notes
% bei `Verweigern' der Datenspende gibt es keine Infos, sondern man wird einach wieder in die Auswahl der verschiedenen Wearbales (in der App, siehe Screenshot) weitergeleitet
% Screenshots lade ich in Seafile hoch
%%------------------------------------------------------------%%
%\input{2_related_work}




% \subsection{What Does Motivate People to Participate in Citizen Science?}

%A critical topic when it comes to citizen science is the motivation of volunteers/contributors and their engagement~\cite{kim2011creek}. This is not only limited to getting involved and starting to participate, but also regards long-term engagement and use of the system~\cite{rotman2012dynamic} for the duration of the project. There are different ways to motivate citizen scientists; some of these strategies include gamification for long-term engagement~\cite{iacovides2013games}, as well as progress information, feedback, attribution and community involvement~\cite{iacovides2013games}~\cite{rotman2012dynamic}. Rotman et al’s findings~\cite{rotman2012dynamic} also point out a difference in the motivational factors with regards to initial motivation to participate, and the long-term one.

%Citizen science can be employed in a variety of disciplines, such as biology~\cite{sullivan2009ebird}, environmental studies~\cite{kim2011creek}, and mathematics~\cite{cranshaw2011polymath}, with applications ranging from observation documentation~\cite{eBird} and data collection and analysis~\cite{zooniverse}, to content creation~\cite{nationalparksservice} and curation~\cite{encyclopediaOfLife}. Regarding data collection in citizen science in particular, it was traditionally analogue, e.g. the National Audubon Society’s community science bird project~\cite{nationalaudubonsociety}. Nowadays, technology has caused a paradigm shift, with data collection primarily taking place on digital platforms~\cite{kim2011creek}. Ubiquitous computing technologies, such as smartphones and smart wearables (e.g. fitness trackers), have rendered digital platforms more accessible and can simplify data collection for citizen scientists, as these devices can be efficiently used as tools for the "fieldwork”.

%Participation in the context of CS can be categorized depending on the “task granularity” required of volunteers~\cite{benkler2006wealth, nov2011technology}. Passive participation occurs with a low granularity contribution, such as in volunteer computing, while in active participation volunteers engage not only in monitoring, but also in analysis. The CDA belongs in the passive participation category, while an example of active participation is Galaxy Zoo (www.galaxyzoo.org), a project in which volunteers analyze images of interstellar dust particles).

%%%% not sure if this paragraph should go here or in the intro%%%%%%

%\subsection{Digital tools for pandemic control using Citizen Science principles}

% - Citizen Science
% - Motivation für Daten teilen (besondere Situation einer Pandemie)
% %- politische Maßnahmen -> Ratings (separates Paper?)
% - there is a need to study `lived experience' of such projects (cf. Enjoying Machines from B. Brown)

% - citizen science allows people to help solve problems that are relevant for or of interest to them (Kim et al., 2011)

% - most citizen science projects are contributory projects (Rotman et al., 2012) 

% - Corona-Data-Donation-App is a contributory project, based on definition from Bonney et al. (2009)

% - citizen scientists participate as collaborators in a scientific research project [REF], volunteer work
% - they perform a more active role compared to other scientific research studies involving members of the public as subjects for example
% - citizen science projects incorporate members of the public enabling data collection on a larger scale over a wider geographical area (term "crowdsourced data" used by covidnearyou.org)
% - and collection of data in certain locations => Corona-Data-Donation-App aims for an exhaustive data collection across Germany (only?) to gain a geographically differentiated view into the spread of COVID-19 in communities, ("importance of physical environment to participation" (Wiggins and Crowsten)~\cite{Wiggins2011})

% - citizen science data collection was traditionally analogue (e.g. National Audubon Society (2010), Christmas Bird Count. birds.audubon.org/history-christmas-bird-count) but is happening mainly on digital platforms today (Kim et al., 2011), ubiquitous computing technologies such as smartphones or fitness tracker/smart wearables make digital platforms more accessible and simplify data collection for citizen scientists, devices can be used as a tool for the "fieldwork"

% - add some examples


% - citizen science applied in a variety of disciplines (cf. Rotman et al., 2012 for references)
% - primary objectives of citizen science projects differ, Corona-Data-Donation-App would be associated as an \textit{investigation project} which focuses on data collection from the physical environment (Kann man Menschen als Teil der Umwelt verstehen? :D) (Wiggins and Crowsten)~\cite{Wiggins2011}, maybe data collection from the "physical" place/community 


% - volunteer motivation and engagement big topics when it comes to citizen science (cf. Kim et al., 2011 for example references)
% - motivation to get involved, initially start participating and use the system, further, motivation to stay engaged for the duration of the project and use system in the long-term
% - initial decision to participate versus long-term engagement (Rotman et al., 2012)
% - citizen scientists often producers and consumers (cf. Kim et al., 2011 for references) => but in this case they are not, or at least not in the short run
% - long-term engagement essential for Corona-Data-Donation-App
% - different ways to motivate citizen scientists (e.g. gamification for long-term engagement: EA Iacovides et al., 2013)
% - recognition and feedback are, amongst others, very important to volunteers (Rotman et al., 2012) cf. for other exemplary strategies
% - progress information and feedback are important (Iacovides et al., 2013)
% - but what about UX?
% - we assume that, during a pandemic, the motivation to participate in citizen projects that address the crisis is relatively high. However, we do not know this for certain. Hence, the need to explore the lived experience of a citizen science project that focuses on the pandemic is needed.

% => citizen science projects are socio-technical and, therefore, social aspects should be considered during the design and development process (Sturm et al. 2018 ~\cite{Sturm2018} (maybe find a better ref)) (maybe refer to the fact that Corona-Data-Donation-App requires smart wearables which automatically narrows the possible user group to a certain proportion of the population)
% - add explanation of socio-technical
% - workshop paper with practical recommendations for the design of mobile apps and platforms for citizen science systems and ethical aspects (Sturm et al. 2018 ~\cite{Sturm2018}), design recommendations include, e.g., ease of use, motivation, "participants journey", available technologies of people (in our case fitness tracker), physical ability (in our case the app is more likely to target athletic people), prevent bias, tech support communication, respect data privacy




% With the rise of COVID-19 cases globally, many countries released digital tools to mitigate the effects of the pandemic. In Germany, the federal government agency Robert Koch Institute responsible for disease control released the \textit{Corona-Datenspende-App} in April 2020. The app uses a citizen science approach to establish an early warning system with data from fitness trackers and smartwatches to detect local fever outbreaks potentially associated with COVID-19. In this paper, we explore the sociopsychological processes and motivations to share such personal data in a citizen science project during a pandemic with personal significance. We analyzed XXX app reviews from the first XX weeks after release and conducted interviews with 10 users to find out how the perception of the pandemic impacted individuals' persistence in using the app. Our findings indicate that users overcame the app's deficiencies through peer support, patience for updates, and perceiving their donation as a unique opportunity to contribute in the fight against COVID-19. Moreover, we observed that the criticised in-transparent use of data did not prevent usage in many cases due to the importance of the matter and the credibility of the RKI. % 183 words atm 
% Concludiung statement that goes beyond a single app. 


%Due to the COVID-19 pandemic, many countries released digital tools to mitigate the effects of this global health crisis. Germany released a virtual citizen science (VCS) project in form of a mobile app that collects fitness tracker data to establish an early warning system for COVID-19, the \textit{Corona-Datenspende-App}. While the HCI community analysed the intricacies of VCS projects from a variety of different angles, our understanding of VCS projects with this level of personal significance is still limited. Most HCI work on VCS focused on topics that were of interest for the respective citizen scientists, but of less personal relevance for them. Consequently, there is a need to build an in-depth understanding of the sociopsychological processes of such VCS projects. To that end, we conducted interviews with 10 users of the app and analysed XXXX online reviews. Based on our analysis we identified a unique set of motivations and actions in the context of VCS. We contribute design implications for future VCS tools in times of crisis that embed user needs and offer long-term engagement. 
